Informatiekunde -- Visie 2003

This document discusses (in Dutch) the vision underlying the business informatics (Informatiekunde) curriculum and research programme at the Nijmegen Institute for Informatics and Information Science (NIII). The ultimate aim of this document is to provide a 'repository' with regard to these visions, and a basis for the specific structure of the program's curriculum and research plans. Since business informatics is a relatively new area for teaching and research at NIII, the current (2003) version of this document primarily focuses on the educational perspective. It is to be expected that in the coming years, updates to this document will also pay more attention to business informatics research. The fact that this document can be updated annually does not mean, however, that we expect an annual change of course. The ambition with regard to the stability of what is described in this document is 5 to 6 years. In the current version, this applies specifically to the vision of the information science study program. The research part of this document will have to be fleshed out even more specifically in the coming years.

==> Images/Aspecten.tex <==
\begin{picture}(16,16)
  \put(3.44,0.75){\Image{width=9.01\unitlength}{DaVinci}}
  \put(0,0){\Image{width=16\unitlength}{AspectenPDF}}
\end{picture}



==> pub.tex <==
{\sc Published as:}
\begin{quote}
  V.~{Kamphuis}, H.A.~(Erik) {Proper}, and S.J.B.A. {Hoppenbrouwers}. {\em {Informatiekunde 2003 -- Visie}}. Nijmegen Institute for Information and Computing Sciences, University of Nijmegen, Nijmegen, The Netherlands, EU, 2003. In Dutch.
\end{quote}

